Rewriting modulo symmetric monoidal structure

String diagrams are a powerful and intuitive graphical syntax for terms of symmetric monoidal categories (SMCs). They find many applications in computer science and are becoming increasingly relevant in other fields such as physics and control theory. An important role in many such approaches is played by equational theories of diagrams, typically oriented and applied as rewrite rules. This paper lays a comprehensive foundation of this form of rewriting. We interpret diagrams combinatorially as typed hypergraphs and establish the precise correspondence between diagram rewriting modulo the laws of SMCs on the one hand and double pushout (DPO) rewriting of hypergraphs, subject to a soundness condition called convexity, on the other. This result rests on a more general characterisation theorem in which we show that typed hypergraph DPO rewriting amounts to diagram rewriting modulo the laws of SMCs with a chosen special Frobenius structure. We illustrate our approach with a proof of termination for the theory of non-commutative bimonoids.

==> source/confBialg.tex <==
% -*- root: ../rewriting.tex -*-

Before proceeding to the confluence proof, we need to develop a bit of critical pair theory for convex rewriting. For simplicity of the presentation, we will only consider \textit{left-mono} rules, i.e. rules $L \xleftarrow{a} i + j \xrightarrow{b} R$ where $a$ is mono. This means, for instance, that identities are excluded from the LHS of a rewrite rule.

\begin{defn}\label{def:critical-pair}
  Consider a convex rewrite system $\mathcal R$ containing a pair of left-mono rewrite rules:
  \[ L \xleftarrow{a} i + j \xrightarrow{b} R \qquad\qquad L' \xleftarrow{a'} i' + j' \xrightarrow{b'} R' \]
  a \textit{critical pair} consists of a hypergraph $H$ and a pair of convex matchings $f : L \to H$ and $f' : L' \to H$ such that:
  \begin{enumerate}
    \item[(i)] $[f,f'] : L + L' \to H$ is epi, and
    \item[(ii)] the induced morphism from the pullback of $(a \poi f, a' \poi f')$ to the pullback of $(f,f')$ is not an isomorphism.
  \end{enumerate}
\end{defn}

Condition (i) states that $L$ and $L'$ should cover $H$, and condition (ii) that they should overlap non-trivially (i.e. not just on their boundary). Already condition (i) is enough to guarantee that there exist finitely many critical pairs for a certain $L$, $L'$.

Let $H', H''$ be the graphs obtained by rewriting $H$ in \eqref{def:critical-pair} using the two distinct matchings $f, f'$. We say $H$ is \textit{joinable} in $\mathcal R$ if it is possible to rewrite $H'$ and $H''$ into isomorphic cospans using the rules in $\mathcal R$.

\begin{defn}
  A convex rewrite system $\mathcal R$ is \textit{locally confluent} if for any $n \rightarrow G \leftarrow m$, and any single-step rewrites $G \rigidDPOstep{\mathcal{R}} G'$ and $G \rigidDPOstep{\mathcal{R}} G''$ it is possible to rewrite $G'$ and $G''$ into isomorphic cospans using the rules in $\mathcal R$.
\end{defn}

By Newman's Lemma~\cite{Baader1998}, any rewrite system that is locally confluent and terminating is confluent, and hence has unique normal forms. So, how do we lift join-ability of critical pairs to local confluence? If we have $G \rigidDPOstep{\mathcal{R}} G'$ and $G \rigidDPOstep{\mathcal{R}} G''$, then its either the case that the images of the matchings $f$, $f'$ which produced these rewrites have no non-trivial overlap (i.e. they are `parallel-independent'~\cite{HandbookGrammar1997}), in which case they are trivially joinable, or the subgraph $H := \im(f) \cup \im(f')$ yields a critical pair.

Suppose we rewrite $H' \rigidDPOstep{\mathcal{R}} H'_1$ at a matching $f$, with a rule $L \leftarrow i+j \rightarrow R$. Then if the embedding $e : H' \to G'$ is convex, then so too is $e \poi f$, so we can lift the rewrite on $H'$ to a rewrite on $G'$:
\begin{equation}\label{eq:cp-lift}
  \xymatrix{
L \ar[d]_f &
i + j
  \ar@{}[dl]|(.8){\text{\large $\urcorner$}}
  \ar@{}[dr]|(.8){\text{\large $\ulcorner$}}
  \ar[l] \ar[r] \ar[d] &
R \ar[d] \\
H' \ar[d]_e &
C \ar@{}[dl]|(.8){\text{\large $\urcorner$}}
  \ar@{}[dr]|(.8){\text{\large $\ulcorner$}}
  \ar[l] \ar[r] \ar[d] &
H'_1 \ar[d]^{e_1} \\
G' & D \ar[l] \ar[r] & G'_1
}
\end{equation}
and furthermore, we have a convex embedding $e_1 : H'_1 \to G'_1$.
Hence we can lift a sequence of rewrites from $H'$ to $G'$. In particular, we can lift the sequence of rewrites that joins $H'$ and $H''$:
\[ H' \rigidDPOstep{\mathcal{R}} H'_1 \rigidDPOstep{\mathcal{R}} H'_2 \rigidDPOstep{\mathcal{R}} \cdots \rigidDPOstep{\mathcal{R}} K \]
\[ H'' \rigidDPOstep{\mathcal{R}} H''_1 \rigidDPOstep{\mathcal{R}} H''_2 \rigidDPOstep{\mathcal{R}} \cdots \rigidDPOstep{\mathcal{R}} K \]
...to one that joins $G'$ and $G''$:
\[ G' \rigidDPOstep{\mathcal{R}} G'_1 \rigidDPOstep{\mathcal{R}} G'_2 \rigidDPOstep{\mathcal{R}} \cdots \rigidDPOstep{\mathcal{R}} M \]
\[ G'' \rigidDPOstep{\mathcal{R}} G''_1 \rigidDPOstep{\mathcal{R}} G''_2 \rigidDPOstep{\mathcal{R}} \cdots \rigidDPOstep{\mathcal{R}} M \]

However, there is a (not so) little subtlety here: the embedding of $H'$ into $G'$ need not be convex. However, in nice cases it is:

\begin{defn}
  A $i \rightarrow H \leftarrow j$ is called \textit{strongly convex} if for any monogamous, acyclic hypergraph $G$, any embedding $e : H \to G$ is convex.
\end{defn}

There is an easy way to characterise strongly convex cospans:

\begin{lem}
  $i \rightarrow H \leftarrow j$ is strongly convex if any only if there is at least one path from each of its inputs to each of its outputs.
\end{lem}

\begin{proof}
  Suppose there exists one path from every input to every output in $H$, and $H \subseteq G$. Then let $p$ be a path in $G$ from a vertex in $H$ to another vertex in $H$ and suppose this path contains a hyperedge not in $h$. Then, the path must pass out an output $y$ of $H$ and in an input $x$ of $H$, which means there must exist a path from $y$ to $x$. However, there must already be a path from $x$ to $y$, so this would violate acyclicity of $G$. Hence $H$ must be convex. Conversely, if there is not a path from an input $x$ to an output $y$, then we can make a monogamous acyclic graph $H'$ by adding a new hyperedge to $H$ with $y$ as its source and $x$ as its target. Then $H$ is not convex in $H'$.
\end{proof}

If the hypergraph associated to a critical pair is strongly convex, the embedding in \eqref{eq:cp-lift} is automatically convex, so the following is immediate:

\begin{thm}
  A convex rewrite system $\mathcal R$ is locally confluent if all of its critical pairs are strongly convex and joinable.
\end{thm}


From this, we have the necessary theory in place to do critical pair analysis on \BA{}. Enumerating the critical pairs for \BA{} gives 34 distinct critical pairs (see Fig.~\ref{fig:cp}), all of which are strongly convex and joinable. For example, here is the joining of the single critical pair between \BA{1} and \BA{9}:
\[
\cgr[height=3.2cm]{critical}
\]



\begin{figure*}\caption{Critical pairs for \BA{}\label{fig:cp}}
  \medskip
  \centering
  \begin{tabular}{rcccccccccc}
          & \BA{1} & \BA{2} & \BA{3} & \BA{4} & \BA{5} & \BA{6} & \BA{7} & \BA{8} & \BA{9} & \BA{10} \\
   \BA{1} &    2   &   0    &   1    &    0   &    2   &    0   &    0   &    1   &    1   &    0    \\
   \BA{2} &        &   2    &   0    &    1   &    0   &    2   &    1   &    0   &    1   &    0    \\
   \BA{3} &        &        &   1    &    0   &    1   &    0   &    0   &    1   &    1   &    0    \\
   \BA{4} &        &        &        &    1   &    0   &    1   &    1   &    0   &    1   &    0    \\
   \BA{5} &        &        &        &        &    1   &    0   &    0   &    1   &    1   &    0    \\
   \BA{6} &        &        &        &        &        &    1   &    1   &    0   &    1   &    0    \\
   \BA{7} &        &        &        &        &        &        &    1   &    0   &    0   &    0    \\
   \BA{8} &        &        &        &        &        &        &        &    1   &    0   &    0    \\
   \BA{9} &        &        &        &        &        &        &        &        &    1   &    0    \\
  \BA{10} &        &        &        &        &        &        &        &        &        &    1    \\
\end{tabular}
\end{figure*}
% counting one trivial critical pair with itself for everything --- 34 critical pairs (24 not counting self-match)


==> source/terminationHopf-old.tex <==



\bR XXXXXXXXXX \e

Let $\mathcal C = \{ C_k \}$ be the set of maximal connected sub-hypergraphs consisting just of $\nu$-hyperedges, and for any path $p$, let $\mathcal C[p] \subseteq \mathcal C$ be the subset consisting just of those $C_k$ which contain a hyperedge from $p$. Then, let:
\[ l_{\mathcal C}(p) := \sum_{C \in \mathcal C[p]} |C| \]
and let the $\mathcal C$-distance from a hyperedge $h$ to a sub-hypergraph $H$ be:
\[ d_{\mathcal C}(h,H) := \max_{p\in\textrm{paths}(h,H)} l_{\mathcal C}(p) \]

For $\textrm{sink}(G)$ be the smallest sub-hypergraph of $G$ containing all outputs and hyperedges of type $\eta$, fix the following sets of hyperedges:
\begin{align*}
  \overline{\mu_k} & := \{ h \ :\  \tau(h) = \mu, d_{\mathcal C}(h, \sink{G}) = k\} \\
  \overline{\nu} & := \{ h \ :\  \tau(h) = \nu \} \\
  \overline{\eta} & := \{ h \ :\  \tau(h) = \eta \} \\
  \overline{\epsilon} & := \{ h \ :\  \tau(h) = \epsilon \} \\
\end{align*}

Let $\leq_{\mathcal C}$ be lexicographic ordering given by:
\[ [\,|\overline{\mu_k}|, |\overline{\mu_{k-1}}|, \ldots, |\overline{\mu_1}|, |\overline{\nu}|, |\overline{\eta}|, |\overline{\epsilon}|\,] \]

\begin{lem}
  The rules {\rm $\HC{j}$} and their converse rules are non-increasing in $\leq_{\mathcal C}$.
\end{lem}

\begin{proof}
  Clearly these rules leave the number of hyperedges of each type fixed, so we only need to show that the numbers $|\overline{\mu_k}|$ remain unchanged.

  We now show that for all $\mu$-hyperedges $h$, that its $\mathcal C$-distance can only decrease. First, consider any $\mu$-hyperedge $h$ not in the image of the LHS of \HC{j}. Then, if the path $p$ with minimal $l_{\mathcal C}(p) = k$ does not pass through the LHS of \HC{j}, $l_{\mathcal C}(p)$ is unchanged. Otherwise, it must enter an input of the LHS and exit an output. Consider the contribution to $l_{\mathcal C}(p)$ of the LHS and RHS of each rule for every input/output pair. For \HC{1} and \HC{3}, it is always zero, for \HC{4} it is always 1, and for \HC{2} it is always 2. Hence, if $h$ is not in the image of the LHS, for every $p$ to $\sink{G}$, there must be a corresponding $p'$ to $\sink{G}$ such that $l_{\mathcal C}(p) = l_{\mathcal C}(p')$.

  Now, consider $\mu$-hyperedges in the image of the LHS. The image of the LHS of \HC{1} contains two $\mu$-hyperedges, each with the same $\mathcal C$-distance $k$. Since any path to $\sink{G'}$ must travel through the unique output, the two $\mu$-hyperedges on the RHS also both have $\mathcal C$-distance $k$. Similarly, the $\mathcal C$-distance of the unique $\mu$-hyperedge in \HC{3} remains unchanged, and the remaining rules don't contain $\mathcal C$-hyperedges.

  Hence the rules \HC{j} are non-increasing in $\leq_{\mathcal C}$, and by symmetry, so too are their converses.
\end{proof}

\begin{lem}
  The rules {\rm $\HR{j}$} are strictly decreasing in $\leq_{\mathcal C}$.
\end{lem}


\bR XXXXXX \e





\bR XXXXXX \e

We now turn out attention to a particular rewrite system, namely the system of commutative and cocommutative Hopf algebras (with trivial antipode) given in Fig.~\ref{fig:hopf}.

\begin{defn}
  A maximal path $p$ in $G$ is a path such that if any path $p'$ contains all of the hyperedges in $p$, then $p = p'$. Let $\mathcal P(G)$ denote the set of all maximal paths.
\end{defn}

For any maximal path $p$ in $G$, let $d(G,p)$ be the number of maximal paths in $G$ that share at least one vertex with $p$ (including $p$ itself). Let:
\[ d(G) := \sum_{p \in \mathcal P(G)} d(G,p) \]
Note paths are being counted multiple times. For example, the LHS of the bialgebra rule has 4 maximal paths, and each of these four paths shares a vertex with all 4 paths, so $d(G) = 16$.

% We extend this to a pre-ordering on hypergraphs in the obvious way:
% \[
% G \geq_d H \Leftrightarrow d(G) \geq d(H)
% \]

\begin{defn} \rm
  A pair of cospans:
  \[ n \rightarrow L \leftarrow m \qquad n \rightarrow R \leftarrow m \]
  has a \textit{path-splitting} if there exists an injection $\phi : \mathcal P(G') \to \mathcal P(G)$ with the following properties:
  \begin{enumerate}
    \item $p$ starts at an input $v$ iff $\phi(p)$ starts at an input $v \in n$
    \item $p$ terminates at an output $v$ iff $\phi(p)$ terminates at an output $v \in m$
    \item if $p$ and $p'$ share a hyperedge, then so too do $\phi(p)$ and $\phi(p')$
  \end{enumerate}
\end{defn}

\begin{lem}
  If there exists a 
\end{lem}


% \begin{lem}
%   If there exists a path-splitting $\phi : H \to G$ then $G \geq_d H$.
% \end{lem}


\begin{lem}
  $\geq_p$ is reflexive, transitive, and well-founded.
\end{lem}

\begin{proof}
  Reflexivity and transitivity are immediate, so suppose $G \geq_p G'$ and $G' \not\geq_p G$. Then, either $G'$ has fewer maximal paths than $G$ or their must be at least one pair of paths in $G$ such that $p, p'$ do not share a hyperedge, but $\phi(p), \phi(p')$ do. Hence any infinite descending chain:
  \[ G >_p G_1 >_p G_2 >_p \ldots \]
  would require infinitely many maximal paths in $G$ to share at least one hyperedge, which is not possible.
\end{proof}


\begin{thm}
  $\geq_p$ is a reduction order. That is, if $G \DPOstep{\mathcal{R}} H$ by applying a rule:
  \[ L \leftarrow n + m \rightarrow R \]
  then:
  \[ L \geq_p R \iff G \geq_p H \]
\end{thm}

\begin{proof}
  Clearly any path-splitting from $H$ to $G$ restricts .
  First, we show this path-splitting lifts to a path-splitting $\widetilde\phi : \mathcal P(H) \rightarrow \mathcal P(G)$ in the following way. Either a path $p$ contains no hyperedges from $R$, in which case let $\widetilde\phi(p) = p$, otherwise it factors into three parts:
  \[ p = [h_1, \ldots h_i, h'_1, \ldots, h'_j, h''_1, \ldots, h''_k]  \]
  where $h'_l \in E_R$ and $h_l, h''_l \in E_H \backslash E_R$. Then, $h_i$ is connected to $h'_1$ via an input of $R$ and $h_j'$ to $h_1''$ via an output. Hence, let:
  \[ \widetilde\phi(p) := [h_1, \ldots h_i] + \phi([h'_1, \ldots, h'_j]) + [h''_1, \ldots, h''_k] \]
  which indeed gives a path in $G$. Furthermore, $\widetilde\phi$ is an injection.
\end{proof}

% Maximal paths start at a unit or an input and terminate at a counit or an output. Let $d(G)$ be the number of duplicate maximal paths and $p(G)$ be the number of all maximal paths. Let $\leq_{d,p}$ be the lexicographic order from $(d,p)$.

\begin{pro}
  The Hopf algebra congruences (assoc, coassoc, commute, cocommute) are non-increasing in $\leq_{d}$.
\end{pro}

\begin{proof}
  All of these rules have exactly one path connecting each input/ouput pair on their LHS and their RHS. Hence applying the rewrite induces a bijection between the old paths $p$ in $G$ and new paths $p'$ in $G[L\Rightarrow R]$. For a pair of paths $p,q$, suppose $p$ and $q$ are not duplicating. Then neither of the paths can be in the image of $L$, and hence $p'$ and $q'$ are not duplicating. Thus $d(G,p) \leq d(G[L\Rightarrow R],p')$. Since the total number of paths is preserved, $d(G) \leq d(G[L\Rightarrow R])$.
\end{proof}

\begin{pro}
  The Hopf algebra reductions (copy, cocopy, unit, counit, bone, bialg, hopf) are strictly decreasing in $\leq_{d}$.
\end{pro}

\begin{proof}
  (sketch/incomplete) All of these rules locally decrease the metric. The only slightly tricky one is bialgebra, where $d(L) = 16$ and $d(R) = 12$. What remains to be shown is locally decreasing the metric implies globally decreasing the metric.
\end{proof}


%$$\cgr{associativityR.pdf}$$

$$\xymatrix{ 
{\cgr{associativityLdpo.pdf} } & 4\ar[l] \ar[r] & { \cgr{associativityR.pdf} }  
}$$


$$\xymatrix{ 
2 & 4\ar[l] \ar[r] & 2}$$

% \begin{figure*}\caption{(Co)commutative Hopf algebra with trivial antipode \label{fig:hopf}}
%   \begin{center}
%   $$  \begin{array}{rccrcc}
%       \HC{1} & := & {\xymatrix{ {\cgr{associativityLdpo.pdf} } & 4\ar[l] \ar[r] & { \cgr{associativityR.pdf} }}}  
%       &
%       \HC{2} & := & {\xymatrix{ {\cgr{coassociativityL.pdf} } & 4\ar[l] \ar[r] & { \cgr{coassociativityR.pdf} }}}  
%       \\
%       \HC{3} & := & {\xymatrix{ {\cgr{commutativityL.pdf} } & 3\ar[l] \ar[r] & { \cgr{commutativityR.pdf} }}}  
%       &
%       \HC{4} & := & {\xymatrix{ {\cgr{cocommutativityL.pdf} } & 3\ar[l] \ar[r] & { \cgr{cocommutativityL.pdf} }}}  
%       \\
%       \HR{1} & := & {\xymatrix{ {\cgr{bialgL.pdf} } & 4\ar[l] \ar[r] & { \cgr{bialgR.pdf} }}}  
%             &
%       \HR{2} & := & {\xymatrix{ {\cgr{boneL.pdf} } & 0\ar[l] \ar[r] & {  }}}  
%       \\
%       \HR{3} & := & {\xymatrix{ {\cgr{duplicationunitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{duplicationunitR.pdf} }}}  
%       &
%       \HR{4} & := & {\xymatrix{ {\cgr{duplicationcounitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{duplicationcounitR.pdf} }}}  
%       \\
%       \HR{5} & := & {\xymatrix{ {\cgr{unitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{unitR.pdf} }}}  
%             &
%       \HR{6} & := & {\xymatrix{ {\cgr{counitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{counitR.pdf} }}}  
%       \\
%       \HR{6} & := & {\xymatrix{ {\cgr{hopfL.pdf} } & 2\ar[l] \ar[r] & { \cgr{hopfR.pdf} }}}  
%     \end{array}$$
%   \end{center}
% \end{figure*}


\begin{figure*}\caption{(Co)commutative Hopf algebra with trivial antipode \label{fig:hopf}}
  \begin{center}
  $$  \begin{array}{rccrcc}
      \HC{1} & := & {\xymatrix{ {\cgr{associativityLdpo.pdf} } & 4\ar[l] \ar[r] & { \cgr{associativityR.pdf} }}}  
      &
      \HC{2} & := & {\xymatrix{ {\cgr{coassociativityL.pdf} } & 4\ar[l] \ar[r] & { \cgr{coassociativityR.pdf} }}}  
      \\
      \HC{3} & := & {\xymatrix{ {\cgr{commutativityL.pdf} } & 3\ar[l] \ar[r] & { \cgr{commutativityR.pdf} }}}  
      &
      \HC{4} & := & {\xymatrix{ {\cgr{cocommutativityL.pdf} } & 3\ar[l] \ar[r] & { \cgr{cocommutativityL.pdf} }}}  
      \\
      \HR{1} & := & {\xymatrix{ {\cgr{bialgL.pdf} } & 4\ar[l] \ar[r] & { \cgr{bialgR.pdf} }}}  
            &
      \HR{2} & := & {\xymatrix{ {\cgr{boneL.pdf} } & 0\ar[l] \ar[r] & {  }}}  
      \\
      \HR{3} & := & {\xymatrix{ {\cgr{duplicationunitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{duplicationunitR.pdf} }}}  
      &
      \HR{4} & := & {\xymatrix{ {\cgr{duplicationcounitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{duplicationcounitR.pdf} }}}  
      \\
      \HR{5} & := & {\xymatrix{ {\cgr{unitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{unitR.pdf} }}}  
            &
      \HR{6} & := & {\xymatrix{ {\cgr{counitL.pdf} } & 2\ar[l] \ar[r] & { \cgr{counitR.pdf} }}}  
      \\
      \HR{6} & := & {\xymatrix{ {\cgr{hopfL.pdf} } & 2\ar[l] \ar[r] & { \cgr{hopfR.pdf} }}}  
    \end{array}$$
  \end{center}
\end{figure*}



%\bR
%
%THIS DOESN'T WORK, SINCE ASSOC. ISN'T MONOTONE....
%
%For a hyperedge $h$, define the maximal path length to an input/output as follows:
%\begin{align*}
%  \textrm{in}(h) & := 1 + \max\{ \textrm{in}(p) \ |\  p \textrm{ is a predecessor hyperedge of } h \} \\
%  \textrm{out}(h) & := 1 + \max\{ \textrm{out}(s) \ |\  s \textrm{ is a successor hyperedge of } h \}
%\end{align*}
%where $\max\{\} = 0$. These are well-defined, since we consider hypergraphs that are directed acyclic.
%
%A rule is called path-monotone if, for every pair consisting of an input and an output, the length of the longest path connecting them is non-increasing from the LHS to the RHS. If there is no path, we call this length $0$.
%
%\begin{pro}\label{prop:image}
%  Let $h$ be a hyperedge not occurring in the image of a path-monotone rewrite $L \Rightarrow R$. Then, for $h'$ the corresponding hyperedge in $G[L\mapsto R]$:
%  \[ \textrm{in}(h) \geq \textrm{in}(h') \qquad\qquad
%     \textrm{out}(h) \geq \textrm{out}(h') \]
%\end{pro}
%
%Let $\mu$ be the type of multiply hyperedges and $\delta$ be the type of comultiply. Then let:
%\[ |G| := \sum_{\{ c \ | \ t(c) = \delta \}} 3^{\textrm{in}(c)} + \sum_{\{m \ | \ t(m) = \mu \}}  3^{\textrm{out}(m)} \]
%The Hopf algebra rewrite system is path-monotone, so by Proposition~\ref{prop:image}, we only need to reduce this metric for hyperedges in the image of a given rewrite rule.
%
%We treat associativity and commutativity as congruences, so we just need to show the remaining laws strictly reduce this metric. The only law that doesn't reduce the number of (co)multiplies is the 2-to-4 bialgebra law. Let $r$ and $s$ be the path lengths of the (co)multiply occurring on the LHS of the rule. Then:
%\[
%3^r + 3^s \ \ \leadsto\ \  2 \cdot 3^{r-1} + 2 \cdot 3^{s-1} < 3^r + 3^s
%\]
%...which is why we take 3 and not 2.
%
%\e

